A formalisation of the SPARC TSO memory model for multi-core machine code

SPARC processors have many applications in mission-critical industries such as aviation and space engineering. Hence, it is important to provide formal frameworks that facilitate the verification of hardware and software that run on or interface with these processors. This paper presents the first mechanised SPARC Total Store Ordering (TSO) memory model which operates on top of an abstract model of the SPARC Instruction Set Architecture (ISA) for multi-core processors. Both models are specified in the theorem prover Isabelle/HOL. We formalise two TSO memory models: one is an adaptation of the axiomatic SPARC TSO model, the other is a novel operational TSO model which is suitable for verifying execution results. We prove that the operational model is sound and complete with respect to the axiomatic model. Finally, we give verification examples with two case studies drawn from the SPARCv9 manual.

==> future.tex <==
\section{Future Work}
\label{sec:future}

An important future work on our agenda is to develop a Hoare-style
logic for SPARC machine code. The current framework, which includes
the abstract ISA model and the memory models, provides a solid
foundation for the verification of concurrent machine code. However,
if a program involves a complex control-flow with branches and loops,
it is difficult to use the current models to reason about the
program. A Hoare-style logic is much desired to make the reasoning
task easier. We can take cues from Myreen et al.'s work on Hoare
logic for ARM machine code~\cite{Myreen2007} and Jensen et al.'s
separation logic for low-level code~\cite{Jensen2013}, and develop a
logic for SPARC to reason about concurrent programs. 

In addition to existing Hoare-style logics for machine code, we will
have to deal with concurrency, which often involves treatments for
local variables and global variables.
Rely/Guarantee~\cite{Jones1981,Jones1983} is a suitable solution for
concurrent program verification, as shown in the Isabelle/HOL
framework for high level programs~\cite{Sanan2017}. A Rely/Guarantee
framework with separation logic on top of this work will make the
reasoning in Section~\ref{sec:case} much easier to be formalised.

% Our project also involves verification of hardware designs and
% high-level programs. Another future direction is to connect this work
% with the other parts of our project. This includes two tasks: (1)
% show the correspondence between low-level programs and high-level
% programs; and (2) show the correspondence between instruction
% semantics and the hardware design. The former task can be done by
% refinement: we show that the low-level program refines the
% corresponding high-level program, and properties such as safety are
% preserved downwards. The latter task involves translating the VHDL
% code of the LEON3 processor design to a language that supports
% automated reasoning and verification, and prove that the hardware
% design and the instruction semantics are consistent. For instance, we
% can formalise the VHDL language in Isabelle/HOL, and show that the
% LEON3 design in the Isabelle/HOL VHDL model corresponds to our
% instruction semantics.

Lastly, we plan to extend the current models with other memory access
instructions. The SPARCv8 model~\cite{hou2016} includes all
instructions in the integer unit. However, similar to the x86-TSO
work~\cite{Sewell2010}, our abstraction and memory model omit the
load/store instructions that access bytes, halfwords, and
doublewords, and focus on words (32-bits) only. The main reason why
we current do not consider mixed-size memory access is that the
axiomatic TSO model~\cite{Sindhu1992,sparcv8} considers fixed size
access only, and it is not clear how the semantics of load/store on
other sizes should be. Taking Figure~\ref{fig:tso} as an example, we
are not sure what should be pushed to the store buffer for a store to
a byte instead of a word. Neither do we know the operations to load a
single byte. The store buffer may have to contain store operations of
various sizes, which also complicates the situation. We conjecture
that the correct behaviour for a load byte operation is as follows:
we need to check all operations in the store buffer, if we can find
the most recent store that \emph{contains} the byte, then we extract
the value of that byte for the load. Otherwise, we check in the
memory for the value of that byte. As another example, if the load
operation is on a doubleword, and we can only find a store to one of
the words in the store buffer, then we will have to obtain the value
of the other word from the memory. None of these conjectures are
verified for SPARC processors, and much work is needed to correctly
model these operations, it may even involve enacting new formal
standards for the industry. Existing work on other architectures may
shed light on this issue~\cite{Flur2017}. However, we believe that it
is easier to extend our operational model with mixed-size memory
access, because the model does not describe the concrete behaviours
of the store buffer.

